SAM4MLLM: Enhance Multi-Modal Large Language Model for Referring Expression Segmentation

We introduce SAM4MLLM, an innovative approach which integrates the Segment Anything Model (SAM) with Multi-Modal Large Language Models (MLLMs) for pixel-aware tasks. Our method enables MLLMs to learn pixel-level location information without requiring excessive modifications to the existing model architecture or adding specialized tokens. We introduce an inquiry-based approach that can effectively find prompt points for SAM to perform segmentation based on MLLM. It combines detailed visual information with the powerful expressive capabilities of large language models in a unified language-based manner without additional computational overhead in learning. Experimental results on pubic benchmarks demonstrate the effectiveness of our approach.

==> algorithms/PPG_inference.tex <==
% \begin{algorithm}[h]
% \caption{SAM4MLLM-PPG inference}
% \label{alg:SAM4MLLM-PPG_infernece}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

% \begin{algorithmic}[1]
% \Require Image of dimensions $H\times W\times 3$, TextDescription
% \Ensure BinaryMask of dimensions $H\times W$
% \State Initialize $BinaryMask[H][W]$ to all zeros
% \State Initialize $P\_positive$ and $P\_negative$ as empty sets
% \State $BoundingBox \gets Ask\_MLLM\_for\_bounding\_box(Image, TextDescription)$
% \State $P\_positive, P\_negative \gets Ask\_MLLM\_for\_points(Image, TextDescription, BoundingBox)$
% \State $BinaryMask \gets SAM(Image, BoundingBox, P\_positive, P\_negative)$
% \State \Return $BinaryMask$
% \end{algorithmic}
% \end{algorithm}


%\begin{algorithm}[h]
\begin{algorithm}[!h]
\caption{SAM4MLLM-PPG inference}
\label{alg:SAM4MLLM-PPG_infernece}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithmic}[1]
\Require Image $\img \in \Real^{H\times W\times 3}$, Text description $\textprompt$
\Ensure Binary mask $\mask \in \{0,1\}^{H\times W}$
% \State Initialize mask $\mask \gets \mathbf{0}$
% \State Initialize point queries $\Ppos, \Pneg \gets \{\}, \{\}$
\State $\Bbox \gets \QueryBbox(\img, \textprompt)$
\State $\Ppos, \Pneg \gets \QueryPoints(\img, \textprompt, \Bbox)$
\State $\mask \gets \SAM(\img, \Bbox, \Ppos, \Pneg)$
\State \Return $\mask$
\end{algorithmic}
\end{algorithm}

==> algorithms/PPG_training.tex <==


\begin{algorithm}[!h]
\caption{SAM4MLLM-PPG training}
\label{alg:SAM4MLLM-PPG_training}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithmic}[1]
\Require Training Set $X_{train}$ % Image $\img \in \Real^{H\times W\times 3}$, Text description $\textprompt$
\Ensure Trained MLLM % Binary mask $\mask \in \{0,1\}^{H\times W}$
% \State Initialize mask $\mask \gets \mathbf{0}$
% \State Initialize point queries $\Ppos, \Pneg \gets \{\}, \{\}$
% \State $\Bbox \gets \QueryBbox(\img, \textprompt)$
% \State $\Ppos, \Pneg \gets \QueryPoints(\img, \textprompt, \Bbox)$
% \State $\mask \gets \SAM(\img, \Bbox, \Ppos, \Pneg)$
% \State \Return $\mask$

\For {batch in $X_{train}$}
    \State Image $\img$, GT Mask $\mask_{gt}$, Text description $\textprompt$ $\gets$ batch 
    \State K groups of Points $P$ $\gets$ RandomSample($\mask_{gt}$)
    \State k groups of $P^+$ and $P^-$ $\gets$ \textit{SAM\_as\_filter}($P$)
    \State $\SAMPromptGT \gets $ Format(k groups of $P^+$ and $P^-$)
    \State $\Ppos, \Pneg \gets \QueryPoints(\img, \textprompt, \Bbox)$
    \State $\SAMPromptMLLM \gets $ Format($\Ppos$ and $\Pneg$)
    \State Loss $\gets$ Auto-regression loss ($\SAMPromptGT, \SAMPromptMLLM$)
    \State Loss.step()
\EndFor


\end{algorithmic}
\end{algorithm}

==> algorithms/PQPP_inference.tex <==
% \begin{algorithm}[h]
% \caption{SAM4MLLM-PQPP inference}
% \label{alg:SAM4MLLM-PQPP_infernece}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

% \begin{algorithmic}[1]
% \Require Image of dimensions $H\times W\times 3$, TextDescription
% \Ensure BinaryMask of dimensions $H\times W$
% \State Initialize $BinaryMask[H][W]$ to all zeros
% \State Initialize $P\_positive$ and $P\_negative$ as empty sets
% \State $BoundingBox \gets Ask\_MLLM\_for\_bounding\_box(Image, TextDescription)$
% \State $SamplePoints \gets Sample\_N\_points\_in\_box(BoundingBox)$
% \For{each $Point$ in $SamplePoints$}
%     \State $IsOnObject \gets Ask\_MLLM\_if\_point\_in\_object(Image, TextDescription, Point)$ \Comment{Returns boolean}
%     \If{$IsOnObject$}
%         \State Add $Point$ to $P\_positive$
%     \Else
%         \State Add $Point$ to $P\_negative$
%     \EndIf
% \EndFor
% \State $BinaryMask \gets SAM(Image, BoundingBox, P\_positive, P\_negative)$
% \State \Return $BinaryMask$
% \end{algorithmic}
% \end{algorithm}

%\begin{algorithm}[h]
\begin{algorithm}[!h]
\caption{SAM4MLLM-PQPP inference}
\label{alg:SAM4MLLM-PQPP_infernece}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithmic}[1]
\Require Image $\img \in \Real^{H\times W\times 3}$, Text description $\textprompt$
\Ensure Binary mask $\mask \in \{0,1\}^{H\times W}$
\State Initialize mask $\mask \gets \mathbf{0}$
\State Initialize point queries $\Ppos, \Pneg \gets \{\}, \{\}$
\State $\Bbox \gets \QueryBbox(\img, \textprompt)$
\State $P \gets \SamplePoints(\Bbox)$
\For{$p \in P$}
    % \State $\IsInside \gets \QueryIsInside(\img, \textprompt, p)$ %\Comment{Returns boolean}
    % \If{$\IsInside$}
    \If{$\QueryIsInside(\img, \textprompt, p)$}
        \State Add $p$ to $\Ppos$
    \Else
        \State Add $p$ to $\Pneg$
    \EndIf
\EndFor
\State $\mask \gets \SAM(\img, \Bbox, \Ppos, \Pneg)$
\State \Return $\mask$
\end{algorithmic}
\end{algorithm}

==> algorithms/PQPP_training.tex <==
\begin{algorithm}[!h]
\caption{SAM4MLLM-PQPP training}
\label{alg:SAM4MLLM-PQPP_training}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithmic}[1]
\Require Image $\img \in \Real^{H\times W\times 3}$, Text description $\textprompt$
\Ensure Binary mask $\mask \in \{0,1\}^{H\times W}$
\State Initialize mask $\mask \gets \mathbf{0}$
\State Initialize point queries $\Ppos, \Pneg \gets \{\}, \{\}$
\State $\Bbox \gets \QueryBbox(\img, \textprompt)$
\State $P \gets \SamplePoints(\Bbox)$
\For{$p \in P$}
    % \State $\IsInside \gets \QueryIsInside(\img, \textprompt, p)$ %\Comment{Returns boolean}
    % \If{$\IsInside$}
    \If{$\QueryIsInside(\img, \textprompt, p)$}
        \State Add $p$ to $\Ppos$
    \Else
        \State Add $p$ to $\Pneg$
    \EndIf
\EndFor
\State $\mask \gets \SAM(\img, \Bbox, \Ppos, \Pneg)$
\State \Return $\mask$
\end{algorithmic}
\end{algorithm}

==> tables/grouped_tables.tex <==
\begin{table}[t]
\vspace{-6pt}
\begin{minipage}[t]{0.58\linewidth}
\centering
\caption{Results on ReasonSeg(Zero-Shot).}
\label{tab:results_reasonseg}
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{val}} \\
\cmidrule{2-3}
& gIoU & cIoU \\
\midrule
{\color{gray} LISA-13B [CVPR-24]~\cite{lai2023lisa}} & {\color{gray} 48.9} & {\color{gray} 46.9} \\
% {\color{gray} LISA-13B-LLaVA1.5 [CVPR-24]~\cite{lai2023lisa}} & {\color{gray} 57.7} & {\color{gray} 60.3} \\
OVSeg [CVPR-23] \cite{liang2023open} & 28.5 & 18.6 \\
GRES [CVPR-23] \cite{liu2023gres} & 22.4 & 19.9 \\
X-Decoder [CVPR-23] \cite{zou2023generalized} & 22.6 & 17.9 \\
SEEM [NeurIPS-23] \cite{zou2024segment} & 25.5 & 21.2 \\
\color{black} LISA-7B [CVPR-24]~\cite{lai2023lisa} & 44.4 & 46.0 \\
% \color{black} LISA-7B-LLaVA1.5 [CVPR-24]~\cite{lai2023lisa} & 53.6 & 52.3 \\
% LISA-7B (ft) & 52.9 & 54.0 \\
% LISA-7B-LLaVA1.5 [CVPR-24] ~\cite{yang2023improved} & 53.6 & 52.3 \\
% LISA-7B-LLaVA1.5 (ft) & 61.3 & 62.9 \\
% LISA++-7B-LLaVA1.5 (ft) & 64.2 & 68.1 \\ \hline
\midrule
SAM4MLLM-7B-PPG & \underline{46.1} & \underline{47.9} \\
SAM4MLLM-7B-PQPP & \textbf{46.7} & \textbf{48.1} \\
% SAM4MLLM-8B-PQPP-LLaVA1.6 & 58.4 & 60.4 \\
\bottomrule
\end{tabular}
\label{table:reasonseg}
\end{minipage}
%
\hfill
%
\begin{minipage}[t]{0.4\linewidth}
\centering
\caption{Result on Vision Question Answering}
\label{tab:results_vqa}
\begin{tabular}{lc}
\toprule
\textbf{Method} & \textbf{VQAv2} \\
\midrule
Qwen-VL-Chat-7B \cite{bai2023qwen} & 78.2 \\
% \midrule
SAM4MLLM-7B-PPG  & {\bf 78.7} \\
SAM4MLLM-7B-PQPP & {\bf 78.7} \\
\bottomrule
\end{tabular}
\label{table:abl_point_sampling}
\end{minipage}
\end{table}


\begin{table}[t]
\centering
\caption{Ablation studies of SAM4MLLM-PQPP.}
\vspace{-1.5em}
\begin{subtable}[t]{0.44\linewidth}
\centering
\caption{Effect of point filter threshold.}
\vspace{-.8em}
\label{tab:ablation_point_threshold}
\begin{tabular}{lc}
\toprule
\textbf{Method} & \textbf{RefCOCOg val} \\
\midrule
0.6 & 69.5 \\
0.7 & 70.8 \\
0.8 & 72.2 \\
0.9 & \textbf{74.5} \\
0.95 & 73.8 \\
\bottomrule
\end{tabular}
\label{table:abl_threshold}
\end{subtable}
%
\hfill
%
\begin{subtable}[t]{0.55\linewidth}
\centering
\caption{Effect of point sampling strategy in inference.}
\vspace{-.8em}
\label{tab:ablation_point_sampling}
\begin{tabular}{lc}
\toprule
\textbf{Method} & \textbf{RefCOCOg val} \\
\midrule
5x5 grid (N=25) & \textbf{74.5} \\
6x6 grid (N=36) & 74.4 \\
random sample (N=25) & 73.7 \\
random sample (N=36) & 74.2 \\
\bottomrule
\end{tabular}
\label{table:abl_point_sampling}
\end{subtable}
\compress
\end{table}

==> tables/grouped_tables_ori.tex <==
\begin{table}[t]
\centering
\caption{Results on ReasonSeg(Zero-Shot).}
\label{tab:results_reasonseg}
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{val}} \\
\cmidrule{2-3}
& gIoU & cIoU \\
\midrule
{\color{gray} LISA-13B [arXiv-23]~\cite{lai2023lisa}} & {\color{gray} 48.9} & {\color{gray} 46.9} \\
OVSeg [CVPR-23] \cite{liang2023open} & 28.5 & 18.6 \\
GRES [CVPR-23] \cite{liu2023gres} & 22.4 & 19.9 \\
X-Decoder [CVPR-23] \cite{zou2023generalized} & 22.6 & 17.9 \\
SEEM [NeurIPS-23] \cite{zou2024segment} & 25.5 & 21.2 \\
LISA-7B [arXiv-23]~\cite{lai2023lisa} & 44.4 & 46.0 \\
% LISA-7B (ft) & 52.9 & 54.0 \\
% LISA-7B-LLaVA1.5 [arXiv-23] ~\cite{yang2023improved} & 53.6 & 52.3 \\
% LISA-7B-LLaVA1.5 (ft) & 61.3 & 62.9 \\
% LISA++-7B-LLaVA1.5 (ft) & 64.2 & 68.1 \\ \hline
\midrule
SAM4MLLM-7B-PPG & \underline{46.1} & \underline{47.9} \\
SAM4MLLM-7B-PQPP & \textbf{46.7} & \textbf{48.1} \\
\bottomrule
\end{tabular}
\label{table:reasonseg}
\end{table}

\begin{table}[t]
\centering
\caption{Result on Vision Question Answering}
\label{tab:results_vqa}
\begin{tabular}{l|c}
\hline
\textbf{Method} & \textbf{VQAv2} \\
\hline
Qwen-VL-Chat-7B \cite{bai2023qwen} & 78.2 \\
\hline
SAM4MLLM-7B-PPG  & 78.7 \\
SAM4MLLM-7B-PQPP & 78.7 \\
\hline
\end{tabular}
\label{table:abl_point_sampling}
\end{table}

\begin{table}[t]
\centering
\caption{Ablation on point filter threshold of SAM4MLLM-PQPP}
\label{tab:ablation_point_threshold}
\begin{tabular}{l|c}
\hline
\textbf{Method} & \textbf{RefCOCOg val} \\
\hline
0.6 & 69.5 \\
0.7 & 70.8 \\
0.8 & 72.2 \\
0.9 & \textbf{74.5} \\
0.95 & 73.8 \\
\hline
\end{tabular}
\label{table:abl_threshold}
\end{table}

\begin{table}[t]
\centering
\caption{Ablation on point sampling strategy of SAM4MLLM-PQPP}
\label{tab:ablation_point_sampling}
\begin{tabular}{l|c}
\hline
\textbf{Method} & \textbf{RefCOCOg val} \\
\hline
5x5 grid (N=25) & \textbf{74.5} \\
6x6 grid (N=36) & 74.4 \\
random sample (N=25) & 73.7 \\
random sample (N=36) & 74.2 \\
\hline
\end{tabular}
\label{table:abl_point_sampling}
\end{table}

==> tables/refcoco.tex <==
\begin{table}[ht]
\centering
\caption{Comparison of methods on refCOCO, refCOCO+, and refCOCOg datasets.}
\label{tab:results_res}
{\resizebox{\textwidth}{!}{
\begin{tabular}{l ccc ccc cc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{refCOCO}} & \multicolumn{3}{c}{\textbf{refCOCO+}} & \multicolumn{2}{c}{\textbf{refCOCOg}} \\ 
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-9}
& val & testA & testB & val & testA & testB & val(U) & test(U) \\
\midrule
\emph{\color{gray} LLM based (13B)} \\
{\color{gray}PerceptionGPT-13B [CVPR-24]~\cite{pi2023perceptiongpt}} & {\color{gray} 75.3} & {\color{gray} 79.1} & {\color{gray}72.1} & {\color{gray}68.9} & {\color{gray}74.0} & {\color{gray}61.9} & {\color{gray}70.7} & {\color{gray}71.9} \\
{\color{gray} GSVA-Llama2-13B [CVPR-24]~\cite{xia2023gsva}} & {\color{gray}79.2} & {\color{gray}81.7} & {\color{gray}77.1} & {\color{gray}70.3} & {\color{gray}73.8} & {\color{gray}63.6} & {\color{gray}75.7} & {\color{gray}77.0} \\
\midrule
\emph{traditional methods} \\
MAttNet (CVPR-18)~\cite{yu2018mattnet} & 56.51 & 62.37 & 51.70 & 46.67 & 52.39 & 40.08 & 47.64 & 48.61 \\
STEP [ICCV-19]~\cite{chen2019see} & 60.04 & 63.46 & 57.97 & 48.19 & 52.33 & 40.41 & - & - \\
LSCM [ECCV-20]~\cite{hui2020linguistic} & 61.37 & 64.99 & 59.55 & 49.34 & 53.12 & 43.50 & - & -  \\
VLT [ICCV-21]~\cite{ding2021vision} & 65.65 & 68.29 & 62.73 & 55.50 & 59.20 & 49.36 & 52.99 & 56.65 \\
SeqTR [ECCV-22]~\cite{zhu2022seqtr} & 67.26 & 69.79 & 64.12 & 54.14 & 58.93 & 48.19 & 55.67 & 55.64 \\
CRIS [CVPR-22]~\cite{wang2022cris} & 70.5 & 73.2 & 66.1 & 65.3 & 68.1 & 53.7 & 59.9 & 60.4 \\
LAVT [CVPR-22]~\cite{yang2022lavt} & 72.7 & 75.8 & 68.8 & 62.1 & 68.4 & 55.1 & 61.2 & 62.1 \\
ReLA [CVPR-23]~\cite{liu2023gres} & 73.8 & 76.5 & 70.2 & 66.0 & 71.0 & 57.7 & 65.0 & 66.0 \\
X-Decoder [CVPR-23]~\cite{zou2023generalized} & - & - & - & - & - & - & 64.6 & - \\
PolyFormer-L [CVPR-23]~\cite{liu2023polyformer} & 76.94 & 78.49 & 74.83 & 72.15 & 75.71 & 66.73 & 71.15 & 71.17 \\
VPD [ICCV-2023]~\cite{zhao2023unleashing} & 73.25 & - & - & 62.69 & - & - & 61.96 & - \\
ETRIS [ICCV-2023]~\cite{xu2023bridging} & 71.06 & 74.11 & 66.66 & 62.23 & 68.51 & 52.79 & 60.28 & 60.42 \\
SEEM [NeurIPS-23]~\cite{zou2024segment} & - & - & - & - & - & - & 65.7 & - \\
\midrule
\emph{LLM based (7B)} \\
\color{black}LISA-7B [CVPR-24]~\cite{lai2023lisa} & 74.9 & 79.1 & 72.3 & 65.1 & 70.8 & 58.1 & 67.9 & 70.6 \\
\color{black}PixelLM-7B [CVPR-24]~\cite{ren2023pixellm} & 73.0 & 76.5 & 68.2 & 66.3 & 71.7 & 58.3 & 69.3 & 70.5 \\
\color{black}PerceptionGPT-7B [CVPR-24]~\cite{pi2023perceptiongpt} & 75.1 & 78.6 & 71.7 & 68.5 & 73.9 & 61.3 & 70.3 & 71.7 \\
\color{black}GSVA-7B [CVPR-24]~\cite{xia2023gsva} & {77.2} & 78.9 & {73.5} & 65.9 & 69.6 & 59.8 & 72.7 & 73.3 \\
\color{black}GLaMM-7B [CVPR-24]~\cite{rasheed2023glamm} & {\ul 79.5} & \textbf{83.2} & \textbf{76.9} & {\ul 72.6} & \textbf{78.7} & {64.6} & {\ul 74.2} & {74.9} \\
\midrule
% SAM4MLLM-7B-PPG & 78.0 & 82.1 & 73.0 & 72.4 & 75.6 & 62.8 & 73.3 & 73.9 \\
% SAM4MLLM-7B-PQPP  & {\ul 79.2} & {\ul 82.1} & {\ul 75.1} & \textbf{74.1} & \textbf{79.0} & \textbf{68.6} & \textbf{75.3} & \textbf{76.0} \\
%SAM4MLLM-7B-PPG & \sout{78.0} & \sout{82.1} & \sout{73.0} & \sout{72.4} & \sout{75.6} & \sout{62.8} & \sout{73.3} & \sout{73.9} \\
%SAM4MLLM-7B-PQPP  & \sout{79.2} & \sout{82.1} & \sout{75.1} & \sout{74.1} & \sout{79.0} & \sout{68.6} & \sout{75.3} & \sout{76.0} \\
SAM4MLLM-7B-PPG & 76.2 & 80.1 & 72.0 & 71.2 & 75.9 & 64.3 & {\ul 74.2} & 74.3 \\
SAM4MLLM-7B-PQPP & 77.1 & {80.9} & 72.5 & {71.5} & {76.8} & {\ul 64.7} & \textbf{74.5} & {\ul 75.2} \\
\color{black}SAM4MLLM-7B-PQPP-LLaVA1.6 & \textbf{79.6} & {\ul 82.8} & {\ul 76.1} & \textbf{73.5} & {\ul 77.8} & \textbf{65.8} & \textbf{74.5} & \textbf{75.6}\\
% SAM4MLLM-LLaVA-1.6-8B & 79.8 & 82.7 & 74.7 & 74.6 & 80.0 & 67.2 & 75.5 & 76.4 \\
\bottomrule
\end{tabular}
}}
\compress
\smallcompress
\end{table}
